ALLSTEPS: Curriculum-driven Learning of Stepping Stone Skills

Humans are highly adept at walking in environments with foot placement constraints, including stepping-stone scenarios where the footstep locations are fully constrained. Finding good solutions to stepping-stone locomotion is a longstanding and fundamental challenge for animation and robotics. We present fully learned solutions to this difficult problem using reinforcement learning. We demonstrate the importance of a curriculum for efficient learning and evaluate four possible curriculum choices compared to a non-curriculum baseline. Results are presented for a simulated human character, a realistic bipedal robot simulation and a monster character, in each case producing robust, plausible motions for challenging stepping stone sequences and terrains.

==> image_page_1.tex <==
% \clearpage

% \begin{figure}%
%   \centering
%   \includegraphics[width=0.9\columnwidth]{figure/cassie_up_down_stairs.png}
%   \includegraphics[width=0.9\columnwidth]{figure/cassie_up_down_spiral.png}
%   \caption{The virtual human walk up a turning staircase.}
%   \label{fig:walker_spiral}
% \end{figure}

% % \begin{figure}%
% %   \centering
% %   \includegraphics[width=0.9\columnwidth]{figure/spiral_stairs.png}
% %   \caption{The virtual human walk up a turning staircase.}
% %   \label{fig:walker_spiral}
% % \end{figure}

% \clearpage
